Radon Transform: Dual Pairs and Irreducible Representations

We illustrate the general point of view developed in [SIAM J. Math. Anal., 51(6), 4356-4381] that can be described as a variation of Helgason's theory of dual $G$-homogeneous pairs $(X,\Xi)$ and which allows us to prove intertwining properties and inversion formulae of many existing Radon transforms. Here we analyze in detail one of the important aspects in the theory of dual pairs, namely the injectivity of the map label-to-manifold $\xi\to\hat\xi$ and we prove that it is a necessary condition for the irreducibility of the quasi-regular representation of $G$ on $L^2(\Xi)$. We further explain how the theory in [SIAM J. Math. Anal., 51(6), 4356-4381] applies to the classical Radon and X-ray transforms in $\mathbb R^3$.

==> macro.tex <==
% our macros

% \newcommand{\N}{\mathbb N}
 \newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
% \newcommand{\T}{\mathbb T}

 \providecommand{\scal}[2]{\langle#1,#2\rangle}

% \newcommand{\id}{\operatorname{id}}
% \newcommand{\dime}{\operatorname{dim}}
% \newcommand{\trace}{\operatorname{tr}}
% \newcommand{\vol}{\operatorname{vol}}
% \newcommand{\supp}{\operatorname{supp}}
% \newcommand{\card}{\operatorname{card}}
% \newcommand{\eps}{\varepsilon}
% \newcommand{\wZ}{Z} % Z

\newcommand{\cA}{{\mathcal A}}
% \newcommand{\cB}{{\mathcal B}}
% \newcommand{\cC}{{\mathcal C}}
% \newcommand{\cD}{{\mathcal D}}
% \newcommand{\cE}{{\mathcal E}}
% \newcommand{\cF}{{\mathcal F}}
% \newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
% \newcommand{\cJ}{{\mathcal J}}
% \newcommand{\cK}{{\mathcal K}}
% \newcommand{\cL}{{\mathcal L}}
% \newcommand{\cM}{{\mathcal M}}
% \newcommand{\cN}{{\mathcal N}}
% \newcommand{\cO}{{\mathcal O}}
%\newcommand{\cP}{{\mathcal P}}
 \newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
% \newcommand{\cS}{{\mathcal S}}
% \newcommand{\cT}{{\mathcal T}}
% \newcommand{\cU}{{\mathcal U}}
% \newcommand{\cV}{{\mathcal V}}
% \newcommand{\cW}{{\mathcal W}}
% \newcommand{\cX}{{\mathcal X}}
% \newcommand{\cY}{{\mathcal Y}}
% \newcommand{\cZ}{{\mathcal Z}}

%\newcommand{\D}{{\rm d}}
% \newcommand{\E}{{\rm e}}

% \newcommand{\red}[1]{{\color{red}#1}}
% \newcommand{\blue}[1]{{\color{blue}#1}}
%  \newcommand{\virgolette}[1]{``#1''}
%  \newcommand{\ga}[1]{{\color{cyan}#1}}
%   \newcommand{\fdm}[1]{{\color{purple}#1}}
%  \newcommand{\gray}[1]{{\color{gray}#1}}
%  \newcommand{\fb}[1]{{\color{magenta}#1}} 
 
%  \newcommand{\rev}[1]{{\color{black}#1}}
 
%  \newcommand{\norm}[1]{{\left\Vert {#1}\right\Vert}}
%  \newcommand{\nt}{w}
%  \newcommand{\ct}{c}

